Changing Computing Paradigms Towards Power Efficiency

Power awareness is fast becoming immensely important in computing, ranging from the traditional High Performance Computing applications, to the new generation of data centric workloads. In this work we describe our efforts towards a power efficient computing paradigm that combines low precision and high precision arithmetic. We showcase our ideas for the widely used kernel of solving systems of linear equations that finds numerous applications in scientific and engineering disciplines as well as in large scale data analytics, statistics and machine learning. Towards this goal we developed tools for the seamless power profiling of applications at a fine grain level. In addition, we verify here previous work on post FLOPS/Watt metrics and show that these can shed much more light in the power/energy profile of important applications.

==> models.tex <==
% \section{Model of energy consumption \label{sec:model}}

% In order to better understand current trends in power consumption at the various subsystems of the chip and in order to facilitate the design of better systems we describe here a simple consumption model. We argue that the tools we developed in this work can be
% used to calibrate this model. By no means however do we claim this to be a complete model. We see it as a vehicle to describe trends.
%
% \def\en#1{E_{\text{#1}}}
% \def\po#1{P_{\text{#1}}}
%
% We split the total energy consumption to several parts which we try to
% estimate separately:
% \begin{packed_itemize}
% \item \emph{Idle energy.} Even when the computer is completely idle, it consumes some energy. If we
% denote $\po{idle}$ idle power of the machine and $t$ time of the computation, the consumed
% energy is:
% $\en{idle} = \po{idle} \cdot t.$
% \item \emph{Floating-point unit energy.} We model the energy consumption of FPU as number of flops times
% unit energy cost of one flop:
% $\en{FPU} = \en{flop} \cdot \text{\#flops}.$
% \item \emph{Arithmetic logic unit energy.} Similarly, the energy is unit cost of one operation
% times number of operations:
% $\en{ALU} = \en{alop} \cdot \text{\#alops}.$
% \item \emph{Cache energy.} We model the energy consumption as number of bits transferred
% times unit energy cost of one bit transfer:
% $\en{cache} = \en{cache bit} \cdot \text{\#cache bits}.$
% \item \emph{Memory energy.} We take unit costs of reading and writing into memory and multiply them
% by number of bits which computation writes and reads:
% $$\en{memory} = \en{write} \cdot \text{\#writing} + \en{read} \cdot \text{\#reading}.$$
% \end{packed_itemize}
% Together we get the total energy consumption of the computation as
% $$E = \en{idle} + \en{FPU} + \en{ALU} + \en{cache} + \en{memory}.$$
% For simplicity, we may omit some factors if they are not significant. In the rest of this section we will test these
% simplified assumptions (most of them are widely used in the community).
%
% \heading{Floating-point unit.}
% The floating-point unit of Power7 has 1-flop, 2-flop, 4-flop and 8-flop operations, the last two being
% vector operations. To reach the theoretical peak performance of the chip, it is necessary to use
% vectorized operations. They are not only faster but they also consume less energy (relative to the number
% of flops computed). For a comparison of 1-flop and 2-flop operations energy consumption, see
% \figurename~\ref{pic:flop_energy}. A key observation is that the energy consumption per GFlop decreases when
% the machine is more stressed.
%
% \heading{Arithmetic logic unit.} Energy consumption of ALU is higher than FPU (compared to unit cost
% of operation). Architecture of Power7 allows only to run one ALU operation per cycle. For details,
% see \figurename~\ref{pic:alop_energy}.
%
%
% \heading{Caches.} We have measured transfer of data inside caches, using different sizes of data to
% use different levels of caches. For larger hierarchies, the unit cost is higher and also power is
% slightly higher; see \figurename~\ref{pic:cache_energy}.
%
%
% \begin{figure}[!t]
% \centering
% %\captionsetup[subfigure]{labelformat=empty}
% \subfloat[\label{pic:alop_energy1}]{\includegraphics[width=0.49\textwidth]{energy_paper16_flop_energy.eps}}\hfill
% \subfloat[\label{pic:alop_energy2}]{\includegraphics[width=0.49\textwidth]{energy_paper17_alop_energy.eps}}\\[2ex]
% \subfloat[\label{pic:alop_energy3}]{\includegraphics[width=0.49\textwidth]{energy_paper18_cache_energy.eps}}
% \caption{Range of energy consumption comparisons. (a)~N-Flop operations vs number of threads: the computation reaches $5.6\,$GFlops per core for 1-flop operations and $11.3\,$GFlops per core for 2-flop operations. (b)~Arithmetic operations vs threads: the computation reaches $3\,$GAlops per core for add, $2.76\,$GAlops per core for mul and $3.33\,$GAlops per core for muladd. (c)~Cache types vs number of threads: the speed of transfer is $9.7\,$GB$/$s for L1 cache, $8.2\,$GB$/$s for L2 cache and $7.6\,$GB$/$s for L3 cache.}
% \label{pic:alop_energy}
% \end{figure}
%
%
% %%%\heading{Memory.} {\tt I DON'T HAVE COMPLETELY ACCURATE DATA AND WAS NOT TESTING THIS HEAVILY. Also
% %%%I ignore slightly increased power of CPU, this is based just on data from memory.}
% %%%Average speed of writing is $74.6\,$MB$/$s, of reading is $73.5\,$MB$/$s. For energy consumption, we
% %%%get $197\,$W$\cdot\,$s per GB written to memory and $233\,$W$\cdot\,$s per GB read from memory.
% %%%Compared to caches, unit consumption of memory is more than $200\times$ larger.
% %%%{\tt I don't have data for copying inside memory, but it was not twice as expensive.}
% %%%
% %%%\heading{Comparison of model.} {\tt I don't have any data here, just some suggestions.}
% %%%We could run some tests (some stuff from ESSL for example, some simple things like standard matrix
% %%%times matrix multiplication), using HPC look into number of operation usages, caches, memory and
% %%%then plug into formula. Then I would make some table with measured energy consumption, estimated
% %%%energy consumption and error. Also concerning idle energy, not really sure which one to use
% %%%(probably total?).
%
% All of the measurements above were accomplished by carefully designed software that ensures that only certain parts of the chip
% are employed. This was also verified by inspecting tracing results obtained by the IBM HPM Toolkit. Thus, while stressing L1 cache
% no flops were performed, etc. An interesting observation is that if L1 cache is stressed enough, then it can consume the same amounts of energy as the floating point unit (see Figs \ref{pic:flop_energy} and \ref{pic:cache_energy}). This is a finding that confirms the projected term of the memory (data movement in general) subsystems to consume much more than the floating point units in future systems.



